Extensions des modules de dimension finie pour les alg\`ebres de courants tordues

Ce m\'emoire traite de la th\'eorie des repr\'esentations d'une certaine classe d'alg\`ebres de Lie de dimension infinie, les alg\`ebres de courants tordues. L'objet du travail est d'obtenir une classification des blocs d'extensions d'une cat\'egorie de modules de dimension finie pour une alg\`ebre de courants tordue donn\'ee. Les principales sources de cette \'etude sont les r\'ecentes classifications des modules simples de dimension finie pour ces alg\`ebres et des blocs d'extensions pour les modules de dimension finie dans le cas des alg\`ebres d'applications \'equivariantes. Ces alg\`ebres de courants tordues comprennent entre autres les familles d'alg\`ebres de Lie des formes tordues et des alg\`ebres d'applications \'equivariantes, donc aussi les incontournables g\'en\'eralisations multilacets, tordues ou non, de la th\'eorie de Kac-Moody affine. / / / / / This master's thesis is about the representation theory of a certain class of infinite dimensional Lie algebras, the twisted current algebras. The object of this work is to obtain a classification of the extension blocks of the category of finite dimensional modules for a given twisted current algebra. The principal motivations for this study are the recent classifications of simple finite dimensional modules for these algebras and of the extension blocks of the category of finite dimensional modules in the case of equivariant map algebras. The class of twisted current algebras includes, amongst others, the families of Lie algebras of twisted forms and equivariant map algebras, therefore the key multiloop generalisations, twisted or not, of the affine Kac-Moody setting.

==> remerciements.tex <==
\chapter*{Remerciements}         % ne pas numéroter
\phantomsection\addcontentsline{toc}{chapter}{Remerciements} % inclure dans TdM

Texte des remerciements en prose.

